Shape of the Cloak: Formal Analysis of Clock Skew-Based Intrusion Detection System in Controller Area Networks

This paper presents a new masquerade attack called the cloaking attack and provides formal analyses for clock skew-based Intrusion Detection Systems (IDSs) that detect masquerade attacks in the Controller Area Network (CAN) in automobiles. In the cloaking attack, the adversary manipulates the message inter-transmission times of spoofed messages by adding delays so as to emulate a desired clock skew and avoid detection. In order to predict and characterize the impact of the cloaking attack in terms of the attack success probability on a given CAN bus and IDS, we develop formal models for two clock skew-based IDSs, i.e., the state-of-the-art (SOTA) IDS and its adaptation to the widely used Network Time Protocol (NTP), using parameters of the attacker, the detector, and the hardware platform. To the best of our knowledge, this is the first paper that provides formal analyses of clock skew-based IDSs in automotive CAN. We implement the cloaking attack on two hardware testbeds, a prototype and a real vehicle (the University of Washington (UW) EcoCAR), and demonstrate its effectiveness against both the SOTA and NTP-based IDSs. We validate our formal analyses through extensive experiments for different messages, IDS settings, and vehicles. By comparing each predicted attack success probability curve against its experimental curve, we find that the average prediction error is within 3.0% for the SOTA IDS and 5.7% for the NTP-based IDS.

==> Sections/acknowledgement.tex <==
\section*{Acknowledgment}
We would like to thank Drs. Sukarno Mertoguno and David Corman for discussions on this problem, and Dr. Kang G. Shin, for his pioneering work that introduced the clock skew-based IDS for automotive CAN networks. This work was supported by NSF grants CNS-1446866 and CNS-1656981, ONR grants N00014-16-1-2710 and N00014-17-1-2946, and ARO grant W911NF-16-1-0485. Views and conclusions expressed are that of the authors and not be interpreted as that of the NSF, ONR or ARO.
